Planting trees in graphs, and finding them back

In this paper we study detection and reconstruction of planted structures in Erd\H{o}s-R\'enyi random graphs. Motivated by a problem of communication security, we focus on planted structures that consist in a tree graph. For planted line graphs, we establish the following phase diagram. In a low density region where the average degree $\lambda$ of the initial graph is below some critical value $\lambda_c=1$, detection and reconstruction go from impossible to easy as the line length $K$ crosses some critical value $f(\lambda)\ln(n)$, where $n$ is the number of nodes in the graph. In the high density region $\lambda>\lambda_c$, detection goes from impossible to easy as $K$ goes from $o(\sqrt{n})$ to $\omega(\sqrt{n})$, and reconstruction remains impossible so long as $K=o(n)$. For $D$-ary trees of varying depth $h$ and $2\le D\le O(1)$, we identify a low-density region $\lambda<\lambda_D$, such that the following holds. There is a threshold $h*=g(D)\ln(\ln(n))$ with the following properties. Detection goes from feasible to impossible as $h$ crosses $h*$. We also show that only partial reconstruction is feasible at best for $h\ge h*$. We conjecture a similar picture to hold for $D$-ary trees as for lines in the high-density region $\lambda>\lambda_D$, but confirm only the following part of this picture: Detection is easy for $D$-ary trees of size $\omega(\sqrt{n})$, while at best only partial reconstruction is feasible for $D$-ary trees of any size $o(n)$. These results are in contrast with the corresponding picture for detection and reconstruction of {\em low rank} planted structures, such as dense subgraphs and block communities: We observe a discrepancy between detection and reconstruction, the latter being impossible for a wide range of parameters where detection is easy. This property does not hold for previously studied low rank planted structures.

==> proofs_line_graphs.tex <==
%
\section{Proofs for planted paths}\label{sec:4}
We say that the ordered set $\{i_1,\ldots,i_K\}$ of $K$ distinct  nodes in $[n]$ is a $K$-path in $G$ if and only if the edges $(i_{\ell},i_{\ell+1})$ are present in $G$ for all $\ell=1,\ldots, K-1$. The previous Lemma \ref{lem:likelihood_ratio} yields, in the case where $\Gamma$ is the line graph, the following 
%%
\begin{lemma}
For planted $K$-path, the likelihood ratio reads
\begin{equation}\label{LR_ll}
L(G):=\frac{\dP_1(G)}{\dP_{0}(G)}=\frac{1}{n(n-1)\cdots(n-K+1)}|\{\hbox{$K$-paths in $G$}\}|\left(\frac{\lambda}{n}\right)^{-K+1}\cdot
\end{equation}
Moreover one has
\begin{equation}\label{LR_lll}
\dE_0(L^2)=\dE_0(x^S),
\end{equation}
where $x=n/\lambda$, and $S$ is a random variable counting the number of edges common to the $K$-path $(1-2-\cdots-K)$ and a random $K$-path $\pi$ chosen uniformly at random among the $n(n-1)\cdots(n-K+1)$ possible ones on node set $[n]$.
\end{lemma}
%%
\begin{proof} Expression \eqref{LR_ll} follows directly from Lemma \ref{lem:likelihood_ratio}.

In the display below, by $\sum_{(i_1\cdots i_K)}$ we mean summation over all the $n(n-1)\cdots(n-K+1)$ oriented paths $(i_1,\ldots,i_K)$ of length $K$ over nodes in $[n]$. Write: 
$$
\begin{array}{lll}
\dE_0(L^2)&=&\sum_{(i_1\cdots i_K)}\sum_{(j_1\cdots j_K)}\left(\frac{(n/\lambda)^{K-1}}{n\cdots(n-K+1)}\right)^2 \dP_0(\hbox{paths }(i_1\cdots i_K)\hbox{ and }(j_1\cdots j_K)\hbox{ present in }G)\\
&=&\sum_{(i_1\cdots i_K)}\left(\frac{(n/\lambda)^{2(K-1)}}{n\cdots(n-K+1)}\right)\dP_0(\hbox{paths }(i_1\cdots i_K)\hbox{ and }(1\cdots K)\hbox{ present in }G)\\
&=&\left(\frac{n}{\lambda}\right)^{K-1}\dP_0(\hbox{ path }\pi=(I_1\cdots I_K)\hbox{ present in }G |\hbox{ path }(1\cdots K)\hbox{ present in }G),
\end{array}
$$
where $\pi=(I_1\cdots I_K)$ is a candidate path chosen uniformly at random from the $n(n-1)\ldots(n-K)$ possible length-$K$ paths. In the above we used symmetry to consider a single path $(1\cdots K)$ instead of all paths $(j_1\cdots j_K)$. 

Note that conditionally on the event that path $(1\cdots K)$ be present in $G$ and on the path $\pi$, the probability that path $\pi$ is also present in $G$ is given by $(\lambda/n)^{K-1-S}$, where $S$ is the number of edges in common between the two paths $\pi$ and $(1\cdots K)$. This yields expression \eqref{LR_lll}.
\end{proof}
%%
%%
%%
%%
\paragraph{Impossibility of detection}
\begin{theorem}
Assume that $\lambda>1$ and $K=o(\sqrt{n})$, or alternatively that $\lambda<1$ and $K=\ln(n)/\ln(1/\lambda)-\omega(\ln(\ln(n)))$. Then the total variation distance $|\dP_1-\dP_0|_{var}$ between $\dP_0$ and $\dP_1$ goes to zero as $n\to \infty$. Thus for any arbitrary test $T(G)\in\{0,1\}$, $\dP_1(T(G)=1)-\dP_0(T(G)=1)\to 0$ as $n\to \infty$.
\end{theorem}
The result follows directly from the 
\begin{lemma}\label{lemma_1}
Assume that $\lambda>1$ and $K=o(\sqrt{n})$, or alternatively that $\lambda<1$ and $K=\ln(n)/\ln(1/\lambda)-\omega(\ln(\ln(n)))$. Then $\lim_{n\to\infty}\dE_0(L^2)=1$.
\end{lemma}
It is standard that the lemma implies the theorem; we reproduce the argument for self-containedness. 
For an arbitrary event $A$, we have by Cauchy-Schwarz inequality
$$
|\dP_1(A)-\dP_0(A)|=|\dE_0((L-1)\II_A)|\le \sqrt{\dE_0((L-1)^2)}.
$$
The right-hand side equals $\sqrt{\dE_0(L^2)-1}$. Since variation distance is the supremum of the left-hand side over events $A$, it is upper bounded by $\sqrt{\dE_0(L^2)-1}$, which by assumption goes to zero as $n\to\infty$.

\begin{proof}(of Lemma \ref{lemma_1}).

We analyze  expression \eqref{LR_lll}.  Set $Z_t=1$ if edge $(I_{t},I_{t+1})$ is part of path $(1\cdots K)$, $Z_t=0$ if it is not part of that path, but $I_{t+1}\in[K]$, and finally $Z_t=-1$ if $I_{t+1}\notin [K]$, so that
\begin{equation}\label{squareLR}
\dE_0(L^2)=\dE_0(x^{\sum_{t=1}^{K-1}Z_t^+})
\end{equation}

Let $\cF_t=\sigma(I_1,\ldots I_t)$, and $n'=n-K$. It is easily verified that we have the following inequalities for all $t=2,\ldots,K-1$:
$$
\dP(Z_t=1|\cF_t)\le\left\{
\begin{array}{ll}
\frac{1}{n'}&\hbox{if }Z_{t-1}=1,\\
\frac{2}{n'}&\hbox{if }Z_{t-1}=0,\\
0&\hbox{if }Z_{t-1}=-1.
\end{array}
\right.
$$
Similarly we have
$$
\dP(Z_t\ge 0|\cF_t)\le \frac{K}{n'}\cdot
$$
Moreover it is easily seen that $\dP(Z_1=1)\le(K/n')(2/n')$, and $\dP(Z_1\ge 0)\le K/n'$.

We now introduce a Markov chain $\{Z'_t\}_{t\ge 1}$ on state space $\{-1,0,1\}$ specified by the initial distribution
$\dP(Z'_1=1)=(K/n')(2/n')$, $\dP(Z'_1\ge 0)= K/n'$ and by the transition probabilities:
$$
\left(
\begin{array}{lll}
1-K/n' & K/n'& 0\\
1-K/n' & (K-2)/n' & 2/n'\\
1-K/n' & (K-1)/n' & 1/n'
\end{array}
\right)
$$
Because of the previous inequalities, we can produce a coupled construction of the two processes $\{Z_t\}$ and $\{Z'_t\}$ such that $Z_1\le Z'_1$, and for $t\ge 1$, if $Z'_t=-1$ then $Z_t=-1$, and furthermore we have the following implications:
$$
\begin{array}{ll}
Z_t=-1 &\Rightarrow Z_{t+1}\le Z'_{t+1},\\
Z_t=Z'_t&\Rightarrow Z_{t+1}\le Z'_{t+1},\\
(Z_t,Z'_t)=(1,0)&\Rightarrow Z_{t+1}\le Z'_{t+1}.
\end{array}
$$
Thus the only situation when we can have $Z_{t+1}>Z'_{t+1}$ is when $(Z_t,Z'_t)=(0,1)$. That is to say, for each time $t+1$ when process $Z$ hits 1 while chain $Z'$ does not, then at time $t$  chain $Z'$ hits 1 while process $Z$ does not.

Because of this, the number of times $t$ at which process $Z$ hits 1 is upper-bounded by the number of times $t$ at which chain $Z'$ does. Thus in view of \eqref{squareLR}, $\dE_0(L^2)$ is upper bounded by $\dE_0 x^{\sum_{s=1}^{K-1}Z'^+_s}$. 


To evaluate this term, introduce the row vector $F(t):=\{f_z(t)\}_{z\in\{-1,0,1\}}$ where $f_z(t):=\dE_0 x^{\sum_{s=1}^tZ'^+_s}\II_{Z'_t=z}$. We then have
\begin{equation}\label{eq:init}
F(1)=(\dP(Z'_1=-1),\dP(Z'_1=0),x\dP(Z'_1=1))=(1-K/n', K/n'(1-2/n'), x(K/n')(2/n')),
\end{equation}
together with the recurrence relation
\begin{equation}\label{eq:iter}
F(t+1)=F(t)M,
\end{equation}
where 
$$
M=\left(\begin{array}{lll}
1-K/n' & K/n' & 0\\
1-K/n' & K/n'-2/n' & x 2/n'\\
1-K/n' & K/n'-1/n' & x/n'
\end{array}
\right)
$$
Recall now that $x=n/\lambda$ and $n'=n-K$, so that $x/n'$ is asymptotic to $1/\lambda$. Thus the above matrix $M$ reads
$$
M=M_0+(K/n)M_1,
$$
where 
\begin{equation}\label{eq:M_0}
M_0=\left(
\begin{array}{lll}
1 & 0 & 0\\
1 & 0 & 2/\lambda\\
1 & 0 & 1/\lambda
\end{array}
\right),
\end{equation}
and the entries of matrix $M_1$ are $O(1)$. Note that $M_0$ admits eigenvalues $0, 1/\lambda,1$ with respective left eigenvectors
$$
\begin{array}{ll}
u_{0}&:=(1,1,-2),\\
u_{1/\lambda}&:=(-\lambda/(\lambda-1),0,1),\\
u_1&:=(1,0,0).
\end{array}
$$
We shall denote $(\mu_{r},v_r)$ the (eigenvalue,eigenvector) pair of  $M$ obtained by perturbation of the eigenpair $(r,u_r)$ of $M_0$, with $r\in\{0,1/\lambda,1)$. By the Bauer-Fike theorem (see \cite{MR1477662}, Theorem VI.25.1) ,  $|\mu_r -r|=O(K/n)$ for all $r$.

Moreover Eq. (1.16), p. 67 in  \cite{Kato:1966:PTL} implies that a normed left (resp., right) eigenvector of $M$ associated to an eigenvalue $\mu_r$ of $M$ differs in norm from a normed left (resp., right) eigenvector of $M_0$ associated to eigenvalue $r$ by $O(K/n)$. We can thus chose $v_r=u_r+O(K/n)$.

Let the decomposition of vector $F(1)$ in the basis provided by the eigenvectors $\{v_r\}$ be given by:
$$
F(1)=\sum_{r\in\{0,1/\lambda,1\}}\alpha_r v_r.
$$
Denote by $e$ the all-ones $3\times 1$ column vector. Our upper bound on $\dE_0(L^2)$ is then given by
\begin{equation}\label{eqn_eig_ub}
\begin{array}{lll}
\dE_0(L^2)&\le & F(K-1) e\\
&=&
F(1)M^{K-2}e\\
&=&\sum_{r\in\{0,1/\lambda,1\}} \alpha_r v_r \mu_r^{K-2} e.
\end{array}
\end{equation}
By our choice of eigenvectors $v_r$ such that $|v_r-u_r|=O(K/n)$, and the fact that 
$$
F(1)=(1+O(K/n))u_{1}+O(K/n)u_{1/\lambda}+O(K/n)u_0,
$$
corresponding weights $\alpha_r$ verify $\alpha_1=1+O(K/n)$, $\alpha_{1/\lambda}=O(K/n)$, $\alpha_0=O(K/n)$. 

In the case where $\lambda>1$ and $K=o(\sqrt{n})$, \eqref{eqn_eig_ub} yields
$$
\dE_0(L^2)\le o(1)+(1+o(1))\mu_1^{K-2}=(1+o(1))(1+O(K/n))^{K-2}\le (1+o(1))e^{O(K^2/n)}.
$$
The assumption that $K=o(\sqrt{n})$ then allows to conclude. 

For $\lambda<1$ and $K=\ln(n)/\ln(1/\lambda) -\omega(\ln(\ln(n)))$, \eqref{eqn_eig_ub} yields
$$
\dE_0(L^2)\le (1+o(1))\left(1+O(K/n)\right)^{K-2}+O(K/n) \left(1/\lambda+O(K/n)\right)^{K-2}.
$$
The first term is $1+o(1))$ since $K^2/n=o(1)$. The second term's logarithm is equivalent to 
$$
\ln(K)-\ln(n)+(K-2)\ln(1/\lambda)\le \ln(\ln(n))-\ln(\ln(1/\lambda))-\omega(\ln(\ln(n))),
$$
and goes to $-\infty$ by assumption. 
\end{proof}
\paragraph{Easiness of detection, dense case}
\begin{theorem}
Assume that $\lambda>1$ and $K=\omega(\sqrt{n})$. Assume that the hidden graph is any connected subgraph on $K$ nodes, not necessarily a line.

Then the total variation distance $|\dP_1-\dP_0|_{var}$ between $\dP_0$ and $\dP_1$ goes to 1 as $n\to \infty$. Furthermore there is a polynomial-time computable test that succeeds with high probability in determining whether an observed graph $G$ is sampled from $\dP_0$ or $\dP_1$.




\end{theorem}
\begin{proof}
Let $k$ denote the size of the hidden connected component, with $k=0$ under $\dP_0$ and $k=K$ under $\dP_1$.

Let $A$ count the number of isolated nodes in $G$, $B$ the number of connected pairs $(i,j)$ that form an isolated component, and $C$ the number of triplets $(i,j,k)$ that form a connected component.

These quantities satisfy with high probability
$$
\begin{array}{ll}
A&=e^{-\lambda}(n-k)+O(\sqrt{n}),\\
B&=\frac{(n-k)^2}{2}\frac{\lambda}{n}e^{-2\lambda}+O(\sqrt{n}),\\
C&=\frac{(n-k)^3}{2}\frac{\lambda^2}{n^2}e^{-3\lambda}+O(\sqrt{n}).
\end{array}
$$
Indeed, only the $n-k$ nodes that are not part of the hidden connected graph can contribute to counts of connected components of size 1, 2 or 3. The above evaluations follow then from evaluation of the expectation and variance of these quantities.

Set $\hat{\lambda}=(nC)/(AB)$. By the previous evaluation,
$$
\hat{\lambda}=\lambda+O(n^{-1/2}).
$$
Now form 
$$
\hat{k}=n-e^{\hat{\lambda}}A.
$$
By the previous evaluations,
$$
\hat{k}=n-(1-O(n^{-1/2}))(n-k)+O(\sqrt{n})=k+O(\sqrt{n}).
$$
The proposed test then decides $H_1$ if $\hat{k}\ge t_n$ and $H_0$ otherwise. Choosing $t_n$ such that $\sqrt{n}\ll t_n \ll K$ then ensures that the test discriminates correctly between the two hypotheses with high probability. For instance, $t_n=\sqrt{K\sqrt{n}}$ works. Necessarily then, the variation distance $|\dP_0-\dP_1|_{var}$ goes to 1 as $n\to\infty$.
\end{proof}
%%
%%
\begin{remark}
If we assume that $\lambda$ is known, a simpler test based on the number of edges in the graph  also succeeds. The test in the above proof still applies even when $\lambda$ is unknown.
\end{remark}
%%
%%
\paragraph{Easiness of detection and reconstruction, sparse case}
Assume $\lambda<1$ and $K=\ln(n)/\ln(1/\lambda)+\omega(1)$. Detection is easy: under $\dP_0$, the expected number of $K$-paths in the graph is $o(1)$, and hence a test which decides $\dP_1$ if there is a $K$-path (which can be found in polynomial time by running depth-first searches) and $\dP_0$ otherwise discriminates the two hypotheses with high probability. 

For reconstruction, assume further that $K=o(n)$. the following algorithm achieves overlap $K(1-o(1))$: construct the longest possible path in $G$; chop its ends so as to reduce it to $K$ nodes. Then with high probability (by the first moment method), the planted path intersects connected components of $G_0$ at most once, and does not intersect connected components of length $\omega(1)$ near its ends. This method must then achieve the announced overlap. [to be detailed]
%%
%%
%%
\section{Impossibility of reconstruction, dense case}
We assume $\lambda>1$ and $K=\omega(\sqrt{n})$. We have seen that with high probability, observation of $G$ allows to determine whether or not an attack has taken place. We now assume that an attack has indeed happened. 


In this context, we shall establish the following result, showing the impossibility of efficient attack reconstruction:
\begin{theorem}
Given $\lambda>1$, $K=\omega(\sqrt{n})$, $K=o(n)$, and a realization $G$ of the graph under $\dP_1$, any estimator $\hat{\cK}$ of the attack achieves negligible overlap, i.e.
$$
\hbox{ov}(\cK)=o(K). 
$$
\end{theorem} 
We first establish a weaker result, namely that necessarily 
\begin{equation}\label{overlap_control_1}
\hbox{ov}(\cK)\le K/2+o(K). 
\end{equation}
This will allow us to introduce the main ideas before we prove the full statement of the theorem.

Fix 
\begin{equation}\label{eq:LD_1}
L=C\ln(n)\hbox{for some suitable constant $C$, } D\gg L\hbox{ and } D^2\ll \frac{n}{\ln(n)}.
\end{equation}  
Condition on the event the attack path is precisely $k_1,\ldots,k_K$. Chop the attack path into $K/(L+D)$ contiguous segments, each of length $M:=L+D$. 

Consider the $\ell$-th segment $\{k_{(\ell-1)M+1},\ldots,k_{\ell M}\}$. We shall construct, for some $I(\ell)\in[(\ell-1)M+1,(\ell-1)M+L]$, a random path of edges in the graph $G$ of the form $k_{I(\ell)},I_2(\ell),I_3(\ell),\ldots,I_{D}(\ell),k_{I(\ell)+D}$ such that none of the nodes $I_2(\ell),\ldots,I_{D}(\ell)$ belong to the attack path, and such that the paths $(k_1,\ldots,k_K)=:k_1^K$ and $k_1^{I(\ell)},I_2^{D}(\ell),k_{I(\ell)+D}^K$ are statistically indistinguishable. More precisely, we have the following:
%%
%%
\begin{lemma}
\label{dvar_control}
%%
%%
There is a construction, for any $\ell\in[K/M]$, of a random path $k_{I(\ell)},I_2(\ell),I_3(\ell),\ldots,I_{D}(\ell),k_{I(\ell)+D}$ such that for any $i\in[(\ell-1)M+1,(\ell-1)M+L]$, any ordered set of $D-1$ distinct nodes $i_2^{D}$ in $[n]\setminus k_1^K$, we have
\begin{equation}\label{eq_dvar_1}
d_{var}(\dP_1(G\in\cdot |\cK=k_1^K,I(\ell)=i,I_2^{D}(\ell)=i_2^{D}),\dP_0(G\in \cdot|k_1^K\in G, (k_i,i_2^{D},k_{i+D})\in G))=\epsilon=o(1).
\end{equation}
This construction moreover verifies the following property. There is an event $\cE$ such that $\dP_1(\cE)=1-o(1)$, and such that, denoting $|I_2^{D}(\ell)\cap I_2^D(\ell')|$ the number of common points between $I_2^{D}(\ell)$ and $I_2^{D}(\ell')$, one has:
\begin{equation}\label{eq_intersections}
 \forall \ell\ne \ell'\in[K/M],\quad \dE_1\left( |I_2^{D}(\ell)\cap I_2^D(\ell')|\II_{\cE}\right) =O\left( \frac{D^2}{n} \right).
\end{equation}
\end{lemma}
%%
%%
Before we prove the Lemma, let us show that it implies \eqref{overlap_control_1}. First, the optimal overlap is achieved by putting in $\hat{\cK}$ the $K$ nodes with the highest probability, conditional on the observed graph $G$, of being in $\cK$. The probability that node $j$ belongs to $\cK$ conditional on $G$ is proportional to the number of $K$-paths in $G$ to which $j$ belongs. This is the so-called ``Maximum a Posteriori'' (MAP) estimation procedure. We denote by $\cK^*$ the corresponding set.  

Second, when under the alternative distribution $\dP_2:=\dP_0(G\in \cdot| k_1^K\in G, (k_i,i_2^{D},k_{i+D})\in G))$ in \eqref{eq_dvar_1}, the joint distribution of the numbers of $K$-paths going through the nodes $k_1^K$ or through the nodes 
in $k_1^i,i_2^{D},k_{i+D}^K$ are statistically indistinguishable. 

Thus, letting $N_{\ell}$ (respectively $N'_{\ell}$) denote the number of points of $k_{(\ell-1)M+1}^{\ell M}$ (respectively, $k_{(\ell-1)M+1}^{i},i_2^{D},k_{i+D}^{\ell M}$) that the MAP estimate selects, one has:
$$
\dE_2(N_{\ell})=\dE_2(N'_{\ell}).
$$
Since each of these variables is bounded by $M=L+D$, the variation distance bound \eqref{eq_dvar_1} implies
$$
\dE_1(N_{\ell})\le \dE_1(N'_{\ell})+\epsilon M.
$$
Summing these inequalities over $\ell\in[K/M]$ yields
\begin{equation}\label{eq_11}
\sum_{\ell=1}^{K/M}\dE_1(N_\ell)=\hbox{ov}(\cK^*)\le\sum_{\ell=1}^{K/M}\dE_1(N'_{\ell})+\epsilon K.
\end{equation}
However, it holds that:
$$
\sum_{i=1}^K\II_{K_i\in\cK^*}+\sum_{j\in\cup_{\ell}I_{2}^{D}(\ell)}\II_{j\in \cK^*}\le K.
$$
This entails (using e.g. Bonferroni's inequality):
$$
\sum_{i=1}^K\II_{K_i\in\cK^*}+\sum_{\ell=1}^{K/M}\sum_{r=2}^{D}\II_{I_r(\ell)\in\cK^*} 
-\sum_{\ell\ne \ell',\ell,\ell'\in[K/M]} |I_2^{D}(\ell)\cap I_2^{D}(\ell')|\le K.
$$
Taking expectations and using the last statement \eqref{eq_intersections} of the Lemma yields, separating evaluations on event $\cE$ and on its complementary set $\overline{\cE}$:
$$
\hbox{ov}(\cK^*)+\sum_{\ell=1}^{K/M}\EE_1(N'_{\ell}) - L(K/M) -(K/M)^2 O(D^2/n) -2 K \dP_1(\overline{\cE})\le K.
$$
Summed with the previous equation \eqref{eq_11}, this gives:
$$
2 \hbox{ov}(\cK^*)\le K + K(\epsilon+(L/M) +(K/n)(D/M)^2+2\dP_1(\overline{\cE})).
$$
The announced result follows from $\epsilon\ll 1$, $L\ll D$, $K=o(n)$  and $\dP_1(\overline{\cE})=o(1)$. 

We now prove Lemma \ref{dvar_control}. 

{\bf Proof of Lemma \ref{dvar_control}, Equation \eqref{eq_dvar_1}: } 
We let $\pi_{i}$ denote the set of candidate paths $k_{i},i_2^{D}(\ell),k_{i+D}$ of the graph, where $i_2^{D}$ are distinct and in $[n]\setminus k_1^K$. For $i\in[(\ell-1)M+1,\ell-1)M+L]$ these can all be used to construct the alternative path in the $\ell$-th segment of $k_1^K$. We denote by
$$
\pi(\ell)=\cup_{i\in[(\ell-1)M+1,\ell-1)M+L]}\pi_{i}
$$
the corresponding collection. Our construction simply amounts to chosing a path uniformly at random from $\pi(\ell)$ in order to construct the alternative path for the $\ell$-th segment, and this independently for each segment. 

Denote $Z_i=|\pi_i|$. Then 
$$
\dE_1(Z_i)=(n-K)(n-K-1)\cdots(n-K-D+2)\left(\frac{\lambda}{n}\right)^D\sim \frac{1}{n}\lambda^D,
$$
since we assumed in \eqref{eq:LD_1} that $D\sim \theta \ln(n)$. Also, by symmetry,
$$
\begin{array}{lll}
\dE_1 Z_i^2 &=& \sum_{i_2^D,j_2^D}\dP_1((k_i,i_2^D,k_i+D)\in G, (k_i,j_2^D,k_{i+D})\in G)\\
&=&\dE_1(Z_i)\sum_{j_2^D}\dP_1((k_i,j_2^D,k_{i+D})\in G| (k_i,i_2^D,k_{i+D})\in G),
\end{array}
$$
where in the last expression we fixed an arbitrary choice $i_2^D$. It follows that:
$$
\dE_1 Z_i^2=(\dE_1(Z_i))^2\dE_1((n/\lambda)^S),
$$
where $S$ is the number of common edges between the fixed path $(k_i,i_2^D,k_{i+D})$ and the path $(k_i,J_2^D,k_{i+D})$ where $J_2^D$ is chosen uniformly at random among $(D-1)$ sequences in $[n]\setminus k_1^K$. 

To control this second moment, we will condition on the number of common edges between the two paths at the beginning and at the end of them, that we shall denote by $X$ and $Y$. These satisfy the constraints $X,Y\ge 0$, $X+Y\le D$. For $X+Y<D$, this forces the choice of $X+Y$ nodes among the $D-1$ to be chosen; for $X+Y=D$, this forces all the $D-1$ choices. Moreover, conditionally on $X,Y$, the expectation of the variable $(n/\lambda)^S$ verifies
$$
\dE_1((n/\lambda)^S|X,Y)\le (n/\lambda)^{X+Y}(1+O(D/n))^D,
$$
by the Markov chain bounds of the previous section. By assumption, $D\ll \sqrt{n}$ so that $(1+O(D/n))^D=1+o(1)$. Thus:
$$
\begin{array}{lll}
\dE_1 Z_i^2&\sim&(\dE_1(Z_i))^2\left[(n/\lambda)^D n^{D-1}+\sum_{x,y\ge 0,x+y<D}(n/\lambda)^{x+y}n^{-(x+y)}(1+o(1))\right]\\
&\le&(1+o(1))[n \lambda^{-D}+(\sum_{x\ge 0}\lambda^{-x})^2]\\
&\le& (1+o(1))\left(\frac{\lambda}{\lambda -1}\right)^2, 
\end{array}
$$
where we used that $n\lambda^{-D}=o(1)$. 

We now evaluate $\dE_1(Z_i Z_j)$ for $i\ne j$. The Markov chain bounding technique of the previous section directly applies to give:
$$
\dE_1(Z_i Z_j)\le (\dE(Z_i))^2(1+o(1)).
$$
Finally we obtain: 
$$
\begin{array}{lll}
\hbox{Var}(|\pi(\ell)|)&=&L \hbox{Var}(Z_i)+\binom{L}{2}\hbox{Cov}(Z_i,Z_j)\\
&\le & \dE_1(Z_i)^2\left[L (1+o(1))\left(\frac{\lambda}{\lambda -1}\right)^2 +L^2 o(1)\right]\\
&\le & \dE_1(|\pi(\ell)|)^2 \left[\frac{1}{L}+o(1)\right].
\end{array}
$$
Since by assumption $L\gg 1$, Tchebitchev's inequality implies that the random variable $|\pi(\ell)|$ concentrates: for some suitable $\epsilon=o(1)$, one has
$$
\dP_1\left(\left|\frac{|\pi(\ell)|}{\dE_1 |\pi(\ell)|}-1\right|\ge \epsilon   \right)\le \epsilon. 
$$
Denote by $\cA$ the event $\cA:=\{|\frac{|\pi(\ell)|}{\dE_1 |\pi(\ell)|}-1|\le \epsilon\}$. It thus has probability at least $1-\epsilon$. Consider a bounded function $f$ of the graph $G$. This concentration result allows us to establish the variation distance bound \eqref{eq_dvar_1} as follows. Write
$$
\dE_1(f(G)|\cA,\cK=k_1^K,I(\ell)=i,I_2^{D}(\ell)=i_2^{D})=\frac{\dE_1[f(G)\II_{\cA}\II_{(k_i, i_2^D,k_{i+D})\in G}\frac{1}{|\pi(\ell)|}]}{\dE_1(\II_{\cA}\II_{(k_i, i_2^D,k_{i+D})\in G}\frac{1}{|\pi(\ell)|})}.
$$
On $\cA$ one has
$$
\frac{1}{\dE_1|\pi(\ell)|}\frac{1}{1+\epsilon}\le \frac{1}{|\pi(\ell)|}\le \frac{1}{\dE_1|\pi(\ell)|}\frac{1}{1-\epsilon}.
$$
This yields:
$$
\frac{1-\epsilon}{1+\epsilon}\frac{\dE_1[f(G)\II_{\cA}\II_{(k_i, i_2^D,k_{i+D})\in G}]}{\dP_1((k_i, i_2^D,k_{i+D})\in G)} \le \dE_1(f(G)|\cA,\cK=k_1^K,I(\ell)=i,I_2^{D}(\ell)=i_2^{D})\le \frac{1+\epsilon}{1-\epsilon}\frac{\dE_1[f(G)\II_{(k_i, i_2^D,k_{i+D})\in G}]}{\dP_1(\cA\cap(k_i, i_2^D,k_{i+D})\in G)}.
$$
By symmetry over all paths in $\pi(\ell)$, denoting by $Z$ the total number of possible paths in it ($Z\sim L n^{D-1}$), one has 
$$
\dP_1(\cA\cap(k_i, i_2^D,k_{i+D})\in G)=\frac{1}{Z}\dE_1(|\pi(\ell)|\II_{\cA}). 
$$
However by definition of $\cA$ this is no smaller than 
$$
\frac{1}{Z}(1-\epsilon)\dE_1|\pi(\ell)| \dP_1(\cA)\ge (1-\epsilon)^2\dP_1((k_i, i_2^D,k_{i+D})\in G).
$$
Finally we obtain:
$$
\begin{array}{l}
\frac{1-\epsilon}{1+\epsilon}\left[\dE_1[f(G)|(k_i, i_2^D,k_{i+D})\in G]-||f||_{\infty}\epsilon\right] \le \dE_1(f(G)|\cA,\cK=k_1^K,I(\ell)=i,I_2^{D}(\ell)=i_2^{D})
\le \cdots \\
\cdots \le 
\frac{1+\epsilon}{(1-\epsilon)^3}\dE_1[f(G)|(k_i, i_2^D,k_{i+D})\in G]
\end{array}$$
{\bf Proof of of Lemma \ref{dvar_control}, Equation \eqref{eq_intersections}}: 
We define the event $\cE$ as, for some suitable constant $\alpha=\Omega(1)$:
\begin{equation}\label{eq_def_cE}
\cE:=\cap_{\ell\in[K/M]}\cE_{\ell},\hbox{ where }\cE_{\ell}:=\{|\pi(\ell)|\ge \alpha \EE_1|\pi(\ell)|\}.
\end{equation}
We then have for arbitrary $\ell\ne \ell'\in[K/M]$:
$$
\dE_1(|I_2^D(\ell)\cap I_2^D(\ell')|\II_{\cE})
=
\sum_{i}\sum_{j}\dE_1\left(\frac{1}{|\pi(\ell)|\cdot|\pi(\ell')|}\sum_{i_2^D\in\pi_i}\sum_{j_2^D\in \pi_j}|i_2^D\cap j_2^D|\II_{\cE}\right)
$$
where the first summations are over  $i\in[M(\ell-1)+1,M(\ell-1)+L]$ and $j\in [M(\ell'-1)+1,M(\ell'-1)+L]$. The expectation in the right-hand side does not depend on $i$ and $j$, by symmetry. Moreover, on $\cE$ we can upper bound the fraction in the expectation by $1/(\alpha\dE_1|\pi(\ell)|)^2$. Thus fixing some arbitrary $i\ne j$:
$$
\begin{array}{ll}
\dE_1(|I_2^D(\ell)\cap I_2^D(\ell')|\II_{\cE})&\le \frac{L^2}{(\alpha\dE_1|\pi(\ell)|)^2}\dE_1\left(\sum_{i_2^D\in\pi_i}\sum_{j_2^D\in \pi_j}|i_2^D\cap j_2^D|\right)\\
&\le 
 \frac{L^2}{(\alpha\dE_1|\pi(\ell)|)^2}\sum_{i_2^D, j_2^D}\dE_1\left(\II_{(k_i,i_2^D,k_{i+D})\in G}\II_{(k_j,j_2^D,k_{j+D})\in G}|i_2^D\cap j_2^D|\right),
\end{array}
$$
where summation is over all pairs of lists $i_2^D$ and $j_2^D$ of $D-2$ distinct elements in $[n]\setminus k_1^K$. Denote by $J_2^D$ one such list selected uniformly at random, and by $i_2^D$ a fixed, arbitrary choice of one such list. One then has, recalling the expression of $\dE_1|\pi(\ell)|=L(\lambda/n)^D (n-K)\cdots(n-K-D+2)$:
\begin{equation}\label{eq:paths_nodes_inter_1}
\dE_1(|I_2^D(\ell)\cap I_2^D(\ell')|\II_{\cE})\le  \frac{1}{\alpha^2}\dE_1\left(\left(\frac{n}{\lambda}\right)^S|i_2^D\cap J_2^D|\right),
\end{equation}
where $S$ denotes the number of edges  in common between the two paths $i_2^D$ and $J_2^D$.


As in the previous section, we now define the Markov chain $\{Z'_t\}_{t\ge 0}$ on the three states $\{-1,0,1\}$, with transition probabilities given by the matrix
$$
P:=\left( 
\begin{array}{lll}
1-D/n' & D/n' & 0\\
1-D/n' & (D-2)/n' & 2/n'\\
1-D/n' & (D-1)/n' & 1/n'
\end{array}
\right),
$$
where $n'=n-K-D$, and with initial condition $Z'_0=-1$. These states are interpreted as follows: $Z'_t=-1$ if $J_{t+1}\notin i_2^D$, $Z'_t=0$ if $J_t\notin i_2^D$ and $J_{t+1}\in i_2^D$, and $Z'_t=1$ if $J_t,J_{t+1}\in i_2^D$. The same coupling argument as before implies, letting $x=n/\lambda$, the following, where the subscript in the second expectation specifies the initial state of the Markov chain $\{Z'_t\}$:
$$
\dE_1\left(\left(\frac{n}{\lambda}\right)^S|i_2^D\cap J_2^D|\right)\le \dE_{-1}\left( x^{\sum_{i=1}^{D-1}Z_i'^+}\sum_{j=1}^{D-1}\II_{Z'_j\ge 0}  \right).
$$
We introduce the notation $F_z(t)=(F_{z,-1}(t),F_{z,0}(t),F_{z,1}(t))$, where 
$$
F_{z,y}(t):=\dE_z\left( x^{\sum_{s=1}^tZ'^+_s}\II_{Z'_t=y}  \right). 
$$
It readily follows that 
$$
F_z(t)=(\II_{z=-1},\II_{z=0},\II_{z=1}) M^t,
$$
where 
$$
M:=\left( 
\begin{array}{lll}
1-D/n' & D/n' & 0\\
1-D/n' & (D-2)/n' & x*(2/n')\\
1-D/n' & (D-1)/n' & x/n'
\end{array}
\right).
$$
This matrix $M$ reads, as previously, $M_0+O(D/n)$ where $M_0$ is given by \eqref{eq:M_0}. Further, $M_0$ admits eigenvalues $0, 1/\lambda,1$ with respective left eigenvectors
$$
\begin{array}{ll}
u_{0}&:=(1,1,-2),\\
u_{1/\lambda}&:=(-\lambda/(\lambda-1),0,1),\\
u_1&:=(1,0,0).
\end{array}
$$
We shall denote $(\mu_{r},v_r)$ the (eigenvalue,eigenvector) pair of  $M$ obtained by perturbation of the eigenpair $(r,u_r)$ of $M_0$, with $r\in\{0,1/\lambda,1)$. By perturbation results (to be filled in), both $|\mu_r -r|$ and $|v_r-u_r|$ are $O(D/n)$. 

Write then, using Markov's property:
$$
\begin{array}{ll}
\displaystyle \dE_{-1}\left( x^{\sum_{i=1}^{D-1}Z'^+_i}\sum_{j=1}^{D-1}\II_{Z'_j\ge 0}  \right)& =
\displaystyle \sum_{j=1}^{D-1}\sum_{z\in\{0,1\}}\dE_{-1}\left( x^{\sum_{i=1}^{j}Z'^+_i}\II_{Z'_j=z}\right)\dE_{z}\left(x^{\sum_{i=1}^{D-j-1}Z'^+_i}  \right)\\
&\displaystyle =\sum_{j=1}^{D-1}\sum_{z\in\{0,1\}} F_{-1,z}(j)\sum_{y=-1,0,1}F_{z,y}(D-j-1).
\end{array}
$$
Perturbation results give the existence of coefficients $[\beta_{z,r}]_{z\in\{-1,0,1\},r\in\{0,1/\lambda,1\}}$ all in $O(1)$ such that
$$
F_z(0)=\sum_{r\in\{0,1/\lambda,1\}}\beta_{z,r} v_r.
$$
It follows that
$$
F_{z}(D-j-1)=\sum_{r\in\{0,1/\lambda,1\}} \beta_{z,r} \mu_r^{D-j-1} v_r=O(1),
$$
since $|\mu_r|\le 1+O(D/n)$ and $D^2\ll n$. It follows that
$$
\begin{array}{ll}
\dE_{-1}\left( x^{\sum_{i=1}^{D-1}Z'^+_i}\sum_{j=1}^{D-1}\II_{Z'_j\ge 0}  \right)&
\displaystyle =\sum_{j=1}^{D-1}F_{-1}(j)\left(\begin{array}{c}0\\1\\1\end{array}\right)\times O(1)\\
&\displaystyle =\sum_{j=1}^{D-1} \sum_{r\in\{0,1/\lambda,1\}}\beta_{-1,r}\mu_r^j v_r\left(\begin{array}{c}0\\1\\1\end{array}\right)\times O(1) .
\end{array}
$$
Since $F_{-1}(0)=u_1$, it holds that $\beta_{-1,1}=1+O(D/n)$, and $\beta_{-1,r}=O(D/n)$ for $r=0,1/\lambda$. The terms with $r=0,1/\lambda$ in the previous expression thus contribute at most $O(D^2/n)$. The terms with $r=1$ give
$$
\sum_{j=1}^{D-1}\beta_{-1,r}\mu_1^j v_1\left(\begin{array}{c}0\\1\\1\end{array}\right)\times O(1)=O(D^2/n),
$$
by using the fact that $v_1=(1,0,0)+O(D/n)$. 

It remains to prove that the event $\cE$ defined in \eqref{eq_def_cE} is such that $\dP_1(\cE)=1-o(1)$. It will suffice to prove that for all $\ell\in[K/M]$, $\dP_1(\cE_{\ell})\ge 1-o(M/K)$. To show this we shall leverage Janson's inequality, as described in \cite{boucheron2013concentration}, p.205, Theorem 6.31. Applied to the random variable $|\pi(\ell)|$, it guarantees that for all $0\le t\le \dE|\pi(\ell)|$ one has
\begin{equation}\label{eq:janson}
\dP_1(|\pi(\ell)|\le \dE|\pi(\ell)|-t)\le e^{-t^2/(2\Delta)},
\end{equation}
where $\Delta$ is the expected number of ordered pairs of paths $(P,Q)$ in $\pi(\ell)$ that share at least an edge. Paralleling our previous bound on the variance of $|\pi(\ell)|$, we distinguish the pairs of paths $(P,Q)$ according to whether they share the same starting point $i\in[(\ell-1)M+1,(\ell-1)M+L]$ or not to write $\Delta=\Delta_1+\Delta_2$, and obtain:
$$
\begin{array}{l}
\Delta_1\le L \frac{\lambda^{2D}}{n^2}(1+o(1))\left(\frac{\lambda}{\lambda-1}\right)^2,\\
\Delta_2\le L^2 \frac{\lambda^{2D}}{n^2}O\left(\frac{D^2}{n}\right).
\end{array}
$$
We moreover have that $\dE|\pi(\ell)|\sim L\frac{\lambda^D}{n}$, so that
$$
\frac{(\dE|\pi(\ell)|)^2}{\Delta}\ge \frac{\Omega(1)}{\frac{1}{L}+\frac{D^2}{n}}\cdot
$$
By our choices \eqref{eq:LD_1} for $L$ and $D$, this lower bound is also $\Omega(1)L=C\Omega(1)\ln(n)$. Taking $t=(1-\alpha)\dE|\pi(\ell)|$ for some $\alpha\in(0,1)$  in \eqref{eq:janson}, we obtain
$$
\dP_1\left(|\pi(\ell)|\le \alpha \dE|\pi(\ell)|\right)\le \exp(-\alpha^2 C\Omega(1)\ln(n)/2).
$$
It readily follows that, for sufficiently large $C$, this probability can be made $o(n^{-3})$ (say), which suffices to conclude the proof of the Lemma.

